Enhancing Adversarial Attacks: The Similar Target Method

Deep neural networks are vulnerable to adversarial examples, posing a threat to the models' applications and raising security concerns. An intriguing property of adversarial examples is their strong transferability. Several methods have been proposed to enhance transferability, including ensemble attacks which have demonstrated their efficacy. However, prior approaches simply average logits, probabilities, or losses for model ensembling, lacking a comprehensive analysis of how and why model ensembling significantly improves transferability. In this paper, we propose a similar targeted attack method named Similar Target~(ST). By promoting cosine similarity between the gradients of each model, our method regularizes the optimization direction to simultaneously attack all surrogate models. This strategy has been proven to enhance generalization ability. Experimental results on ImageNet validate the effectiveness of our approach in improving adversarial transferability. Our method outperforms state-of-the-art attackers on 18 discriminative classifiers and adversarially trained models.

==> Section/old_method.tex <==




% In MI-CSE algorithm, it has been proven that updating using such algorithm equivalent to maximizing the cosine similarity between gradients and the loss function simultaneously:
% \begin{equation}
%     \mathbb{E}[x_t^n - x_t] \approx \beta \mathbb{E}[\sum_{i=1}^n\frac{g_i}{||g_i||_2}] + \frac{\beta^2}{2}\mathbb{E}[\sum_{i < j}\frac{\partial \frac{g_ig_j}{||g_i||_2||g_j||_2}}{\partial x}]
% \end{equation}


% However, the proportion of weights of the $\mathbb{E}[\sum_{i=1}^n\frac{g_i}{||g_i||_2}]$ and $\mathbb{E}[\sum_{i < j}\frac{\partial \frac{g_ig_j}{||g_i||_2||g_j||_2}}{\partial x}]$ are limited to $1 : \frac{\beta}{2}$, making it hard to trade-off between optimization is
% regularization. Besides, this algorithm has $O(\beta^3)$ approximation error, including $\beta$ will cause a larger approximation error, leading to performance degradation.


% In order to get away from the constraints, we find we could first accurately calculate $g_{loss} = \sum_{i = 1}^n \frac{g_i}{||g_i||_2}$ directly during the inner loop iteration, and we use the update $x_t^n - x_t$, which is the update for $x$ after finishing the whole inner loop iteration for one time, minus the loss term to get cosine term $g_{cos} = \sum_{i,j,i<j}\frac{\partial \frac{g_ig_j}{||g_i||_2||g_j||_2}}{\partial x}$. Now, we can combine the loss term and cosine term freely as follows:
% \begin{equation}
%     \mathbb{E}[x_t^n - x_t] = \lambda_1 g_{loss} + \lambda_2 g_{cos}
% \end{equation}


% This help the algorithm get away from the constraints of weights, which not only enable us to arbitrarily regulate the optimization and regularization, but also relieve the influence of the approximation error since we can set $\beta$ to a smaller value, which decrease the $O(\beta^3)$.


% %%%%%%% The derivation of MI-CSE %%%%%%%%%
% Now, we prove the updating process in MI-CSE. we use $p_i$ to denote the closest optimum of the $i^{th}$ model $f_{i}\in \mathcal{F}$ to the adversarial example $x$ and use $H_i$ to denote the Hessian matrix of $L(f_i(x),y)$ at $p_i$. We employ the second order Taylor expansion to approximation (1) at $p_i$:
% \begin{equation}
%     \mathbb{E}_{f_i \in \mathcal{F}}[L(f_i(p_i), y) + \frac{1}{2}(x - p_i)^TH_i(x - p_i)]
% \end{equation}


% Since [12,13] have proven that the local optima have nearly the same value with global optimum in nerual networks, we mainly focus on the second term $\mathbb{E}[\frac{1}{2}(x - p_i)^TH_i(x - p_i)]$. 


% [9] use Cauchy-Swartz theorem and get the upper bound of the second term as:
% \begin{equation}
%     \mathbb{E}[(x - p_i)^TH_i(x - p_i)] \leq \mathbb{E}[||H_i||_F]\mathbb{E}[||(x - p_i)||_2^2]
% \end{equation}


% The first term correspond to the flatness of the landscape, which is a crucial factor for the generalization ability [14-16] and has been adequately explored in [14]. In this work, we mainly focus on $\mathbb{E}[||(x - p_i)||_2^2$. In order to optimize it, [9] derives an upper bound :
% \begin{equation}
%     \frac{1}{|\mathcal{F}_t|}\sum_{i = 1}^n||x - p_i||_2^2 \leq -\frac{2\max{||H_i^{-1}||_F^2}}{n}\sum_{i=1}^n\sum_{j=1}^{i-1}g_ig_j
% \end{equation}


% Where $g_i$ denotes the loss gradient of the surrogate model $i$. Consequently, we find that maximizing the cosine similarity between gradients will result in a better generalization ability.


% In order to optimize this cosine similarity, [9] proposes an approximation algorithm named MI-CSE, which first update $x_i$ with the current gradient $g_{i-1} = \nabla_x L(f_{i-1}(x_{i-1},y))$ in the inner optimization:
% \begin{equation}
%     x_t^i = clip_{x^{real},\epsilon}(x_t^{i-1} + \beta \frac{g_{i-1}}{||g_{i-1}||_2})
% \end{equation}


% Therefore, we can view the update $x_t^n - x_t$, which is the update after a whole inner loop iteration for one time as the approximated gradient for iteration $t$ and then we get the update of $x$ after one outer loop iteration:
% \begin{equation}
%     x_{t + 1} = clip_{x^{real},\epsilon}(x_t + \alpha \dot sign(x_t^n - x_t))
% \end{equation}












% \subsection{Cosine similarity between gradients}


% We use $p_i$ to denote the closest optimum of the $i$th model $f_i\in \mathcal{F}$ to the adversarial example $x$ and use $H_i$ to denote the Hessian matrix of $L(f_i(x), y)$ at $p_i$. We employ the second-order Taylor expansion to approximate \cref{eq:adv_defination} at $p_i$:
% \begin{equation}
% \label{eq:taylor}
%     \mathbb{E}_{f_i\in \mathcal{F}}[L(f_i(p_i),y) + \frac{1}{2}(x-p_i)^TH_i(x-p_i)]
% \end{equation}


% According to \cref{eq:taylor}, we can find that a larger value of $\mathbb{E}[L(f_i(p_i),y)]$ and $\mathbb{E}[(x-p_i)^TH_i(x-p_i)]$ means a better performance. For the first term, \cite{kawaguchi2019every,laurent2018deep} have proven that the local optima have nearly the same value with the global optimum in neural networks. Therefore, we mainly focus on the second term to improve the transferability of adversarial examples.


% \cite{chen2023rethinking} use the Cauchy-Swartz theorem and get the upper bound of the second term as:
% \begin{equation}
%     \mathbb{E}[(x-p_i)^TH_i(x-p_i)]\leq \mathbb{E}[||H_i||_F]\mathbb{E}[||(x-p_i)||_2^2].
% \end{equation}


% The first term correspond to the flatness of the landscape, which is a crucial factor for the generalization ability~\cite{chen2022bootstrap, wei2023relation, wei2023cfa}. And has been adequately explored in~\cite{chen2022bootstrap}. In this work, we mainly focus on $\mathbb{E}[||(x-p_i)||_2^2]$. Since it's hard to directly optimize $\frac{1}{|\mathcal{F}_t|}\sum_{i=1}^{|\mathcal{F}_t|}||x-p_i||_2^2$, \cite{chen2023rethinking} derives an upper bound:
% \begin{equation}
%     \frac{1}{|\mathcal{F}_t|}\sum_{i=1}^{|\mathcal{F}_t|}||x-p_i||_2^2\leq -\frac{2\max||H_i^{-1}||_F^2}{n}\sum_{i=1}^n\sum_{j=1}^{i-1}g_ig_j,
% \end{equation}


% Where $g_i$ is the loss gradient of the surrogate model $i$. Consequently, we find that maximizing the cosine similarity between gradients will result in a better generalization ability.



% \subsection{Derivation of ST}


% However, the cosine similarity between gradients is still hard to optimize. To this end, \cite{chen2023rethinking} proposes an approximation algorithm named MI-CSE, which first update $x_i$ with the current gradient $g_{i-1}=\nabla_x L(f_i(x_{i-1},y)$ in the inner optimization:

% \begin{equation}
% x_{t}^i = clip_{x^{real},\epsilon}(x_t^{i-1} + \beta \frac{g_{i-1}}{||g_{i-1}||_2})
% \end{equation}

% And view the update $x_t^n - x_t$ as the approximated gradient for iteration $t$:


% \begin{equation}
%     x_{t+1} = clip_{x^{real},\epsilon}(x_t + \alpha \cdot sign(x_t^n - x_t))
% \end{equation}


% It has been proven that updating using such algorithm equivalent to maximizing the cosine similarity between gradients and the loss function simultaneously:
% \begin{equation}
%     \mathbb{E}[x_t^n-x_t] \approx \beta \mathbb{E}[\sum_{i=1}^n\frac{g_i}{||g_i||_2}] + \frac{\beta^2}{2}\mathbb{E}[\sum_{i<j}
% \frac{\partial \frac{g_ig_j}{||g_i||_2||g_j||_2}}{\partial x}]
% \end{equation}





% However, the proportion of weights of the $\mathbb{E}[\sum_{i=1}^n\frac{g_i}{||g_i||_2}]$ and $\mathbb{E}[\sum_{\substack{i<j}}
% \frac{\partial \frac{g_ig_j}{||g_i||_2||g_j||_2}}{\partial x}]$ are limited to $1:\frac{\beta}{2}$, making it hard to trade-off between optimization are regularization. Besides, this algorithm has $O(\beta^3)$ approximation error, increasing $\beta$ will cause a larger approximation error, leading to performance degradation.


% In order to get away from the constraints, we find that we could first accurately calculate $g_{loss} = \sum_{i=1}^n\frac{g_ig_j}{||g_i||_2||g_j||_2}$ directly, and we use the update $x_t^n-x_t$ minus the loss term to get the cosine term $g_{cos} = \sum_{\substack{i,j\\i<j}}
% \frac{\partial \frac{g_ig_j}{||g_i||_2||g_j||_2}}{\partial x}$. Finally, we combine them to update as follows:
% \begin{equation}
%     \mathbb{E}[x_t^n-x_t] = \lambda_1 g_{loss} + \lambda_2 g_{cos}
% \end{equation}


% Which gives us more flexibility to trade-off between optimization and regularization.

